PAC-Bayesian Soft Actor-Critic Learning

Actor-critic algorithms address the dual goals of reinforcement learning (RL), policy evaluation and improvement via two separate function approximators. The practicality of this approach comes at the expense of training instability, caused mainly by the destructive effect of the approximation errors of the critic on the actor. We tackle this bottleneck by employing an existing Probably Approximately Correct (PAC) Bayesian bound for the first time as the critic training objective of the Soft Actor-Critic (SAC) algorithm. We further demonstrate that online learning performance improves significantly when a stochastic actor explores multiple futures by critic-guided random search. We observe our resulting algorithm to compare favorably against the state-of-the-art SAC implementation on multiple classical control and locomotion tasks in terms of both sample efficiency and regret.

==> aux.tex <==
\subsection{Representative baselines}
\label{sec:baselines}


We aim to challenge our main hypothesis maximally by exploring the most promising alternative design choices that may improve SAC. To this end, we introduce two representative approaches targeting most similar problems to ours and curate new and maximally competitive baseline models from them. We leave a comprehensive literature survey to Appendix A.1.

{\bf Fitted Policy Iteration (FPI)}\cite{antos2008learning} addresses the relationship between the expected Bellman residual and the risk functional given in Eq. \ref{eq:bias} by a loss function
\begin{align*}
    L_{\mathrm{FPI}}(Q_\pi^\theta;\pi, g) = R_N(\theta;\pi, \mathcal{D}) -\nonumber || g(s_t, a_t) - r(s_t, a_t) - \gamma Q_\pi^\theta (s_{t+1}, a_{t+1}) ||_{p_\pi(s_t) \pi(a_t|s_t)}^2
\end{align*}
that uses an auxiliary function $g$ to neutralize the overestimation bias by solving a minimax problem $\arg \min_{\theta} \max_g L_{FPI}(Q_\pi^\theta;\pi, g)$. The original paper introduces FPI as a solely theoretical contribution. Since the vanilla implementation of this loss is both computationally expensive and unstable, we strengthen it by assuming a randomized critic and adopt soft Bellman backups. We coin the resulting baseline as {\bf SAC-FPI}. Our target model PAC4SAC differs from this baseline by its complexity penalty and the multiple shooting scheme.

{\bf Network Randomization (NR)}\cite{lee2019network} aims to sidestep the effects of value estimation errors by randomizing its actor network input. NR passes the actor inputs through an auxiliary network $f$ with random weights. It enhances the robustness of the actor network by inducing invariance to input perturbation via a regularization term, resulting in the loss function below:
\begin{align*}
  L_{\mathrm{NR}}(\psi)  = \frac{1}{N}\sum_{t=1}^N \Big (- \log \pi (a_t|f(s_t;\phi);\psi) R_t + \nonumber \beta \lVert h(f(s_t;\phi);\psi) - h(s_t;\psi)\rVert^2  \Big),
\end{align*}
where $f$ is a network with randomly generated and not learned parameters $\phi$ that perturbs the input of the actor network $\pi$ parameterized by $\psi$, the coefficient $R_t$ refers to the cumulative reward at time step $t$ and $h$ denotes the output of the penultimate layer of $\pi$. The coefficient $\beta > 0$ is a regularization parameter. The original paper implements this REINFORCE-like loss using the Proximal Policy Optimization (PPO) \cite{schulman2017proximal} design. Our preliminary tries showed significant performance improvement when we use the same randomization scheme in the SAC design, hence train the actor by 
\begin{align*}
    \arg \max_\psi \frac{1}{N}\sum_{t=1}^N ~\mathbb{E}_{\pi(a_t|s_t; \psi)} [Q_\pi^{\theta}(s_t,a_t) - \log \pi(a_t|f(s_t;\phi);\psi)] + \beta \mathbb E_{s_t \in \mathcal{D}} \left[\lVert h(f(s_t;\phi);\psi) - h(s_t;\psi)\rVert^2  \right].
\end{align*}
To the favor of the prior work, we take this version as our baseline and refer to it as {\bf SAC-NR}.

{\bf Optimistic Actor Critic (OAC)\cite{ciosek2019better}} tries to cope with poor sample efficiency of Actor-Critic methods. It defines a probabilistic critic that allows calculation of LCB and UCB, and trains the critic with LCB to mitigate overestimation bias. For action sampling it uses a behavior policy trained on the UCB of the critic and deterministically selects the best action on an optimistic estimate of the state-action value function. This baseline is the closest baseline to our approach, however our model is different from OAC in both critic training and action selection. For training the critic network our model use a principled PAC-Bayesian bound instead. Action selection method in our model is done with multiple shooting technique which is similar to UCB in spirit, but it is empirical.

\begin{figure*}[ht]
    \centering
    \includegraphics[width = 1\linewidth]{fig/results.pdf}
    \caption{Learning curves of PAC4SAC and the baselines. Our PAC4SAC improves the state of the
art in both sample efficiency as visible from the area under episode reward curve scores and asymptotic performance as visible from the
highest rewards. Its consistent improvement over SAC demonstrates the effect of PAC Bayesian critic training on performance.}
    \label{fig:learning-curves}
\end{figure*}

